Second-Order Propositional Satisfiability

Fundamentally, every static program analyser searches for a proof through a combination of heuristics providing candidate solutions and a candidate validation technique. Essentially, the heuristic reduces a second-order problem to a first-order/propositional one, while the validation is often just a call to a SAT/SMT solver. This results in a monolithic design of such analyses that conflates the formulation of the problem with the solving process. Consequently, any change to the latter causes changes to the whole analysis. This design is dictated by the state of the art in solver technology. While SAT/SMT solvers have experienced tremendous progress, there are barely any second-order solvers. This paper takes a step towards addressing this situation by proposing a decidable fragment of second-order logic that is still expressive enough to capture numerous program analysis problems (e.g. safety proving, bug finding, termination and non-termination proving, superoptimisation). We refer to the satisfiability problem for this fragment as Second-Order SAT and show it is NEXPTIME-complete. Finally, we build a decision procedure for Second-Order SAT based on program synthesis and present experimental evidence that our approach is tractable for program analysis problems.

==> synth-benchmarks.tex <==
\section{Benchmarks}
\label{app:benchmarks}

\begin{figure}
\scriptsize
 \begin{multicols}{4}
 
   \begin{minipage}{.2\textwidth}
   \bf{P1}($x$): Turn-off rightmost 1 bit.
   \begin{enumerate}
    \item $t1 = x - 1$
    \item $t2 = x \& t1$
   \end{enumerate}
   \end{minipage}

   \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   \bf{P2}($x$): Test whether $x$ is of the form $2^n - 1$.
   \begin{enumerate}
    \item $t1 = x + 1$
    \item $t2 = x \& t1$
   \end{enumerate}
   \end{minipage}

   \vspace{12pt}
   

   \begin{minipage}{.2\textwidth}
   \bf{P3}($x$): Isolate the rightmost 1 bit.
   \begin{enumerate}
    \item $t1 = -x$
    \item $t2 = x \& t1$
   \end{enumerate}
   \end{minipage}

   \vspace{12pt}
   

   \begin{minipage}{.2\textwidth}
   \bf{P4}($x$): Form a mask that identifies the rightmost 1 bit and trailing 0s.
   \begin{enumerate}
    \item $t1 = x - 1$
    \item $t2 = x \oplus t1$
   \end{enumerate}
   \end{minipage}

   \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   \bf{P5}($x$): Right propagate the rightmost 1 bit.
   \begin{enumerate}
    \item $t1 = x - 1$
    \item $t2 = x \mid t1$
   \end{enumerate}
   \end{minipage}

   \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   \bf{P6}($x$): Turn on the rightmost 0 bit.
   \begin{enumerate}
    \item $t1 = x + 1$
    \item $t2 = x \mid t1$
   \end{enumerate}
   \end{minipage}
      \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   \bf{P7}($x$): Isolate the rightmost 0 bit.
   \begin{enumerate}
    \item $t1 = \sim x$
    \item $t2 = x + 1$
    \item $t3 = t1 \& t2$
   \end{enumerate}
   \end{minipage}
   \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   \bf{P8}($x$): Form a mask the identifies the trailing 0s.
   \begin{enumerate}
    \item $t1 = x -1$
    \item $t2 = \sim x$
    \item $t3 = t1 \& t2$
   \end{enumerate}
   \end{minipage}
   \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   \bf{P9}($x$): Absolute value.
   \begin{enumerate}
    \item $t1 = x >> 31$
    \item $t2 = x \oplus t1$
    \item $t3 = t2 - t1$
   \end{enumerate}
   \end{minipage}

      \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   \bf{P10}($x, y$): Test if nlz(x) == nlz(y), where nlz is number of leading zeroes.
   \begin{enumerate}
    \item $t1 = x \& y$
    \item $t2 = x \oplus y$
    \item $t3 = t2 \leq t1$
   \end{enumerate}
   \end{minipage}

   
      \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   \bf{P11}($x, y$): Test if nlz(x) < nlz(y).
   \begin{enumerate}
    \item $t1 = \sim y$
    \item $t2 = x \& t1$
    \item $t3 = t2 > y$
   \end{enumerate}
   \end{minipage}
   \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   \bf{P12}($x, y$): Test if nlz(x) <= nlz(y).
   \begin{enumerate}
    \item $t1 = \sim y$
    \item $t2 = x \& t1$
    \item $t3 = t2 \leq y$
   \end{enumerate}
   \end{minipage}
   
      \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   \bf{P13}($x$): Sign.
   \begin{enumerate}
    \item $t1 = x >> 31$
    \item $t2 = t1 < x$
    \item $t3 = t2 + t1$
   \end{enumerate}
   \end{minipage}

   \vspace{12pt}

   \begin{minipage}{.2\textwidth}
   \bf{P14}($x, y$): Floor of average of $x$ and $y$ without overflowing.
   \begin{enumerate}
    \item $t1 = x \& y$
    \item $t2 = x \oplus y$
    \item $t3 = t2 >> 1$
    \item $t4 = t1 + t3$
   \end{enumerate}
   \end{minipage}
   \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   \bf{P15}($x, y$): Ceil of average of $x$ and $y$ without overflowing.
   \begin{enumerate}
    \item $t1 = x \mid y$
    \item $t2 = x \oplus y$
    \item $t3 = t2 >> 1$
    \item $t4 = t1 - t3$
   \end{enumerate}
   \end{minipage}
   \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   \bf{P16}($x$): Max.
   \begin{enumerate}
    \item $t1 = x \leq y$
    \item $t2 = x \oplus y$
    \item $t3 = t1 * t2$
    \item $t4 = t3 \oplus y$
   \end{enumerate}
   \end{minipage}
   \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   \bf{P17}($x$): Turn off the rightmost contiguous string of 1 bits.
   \begin{enumerate}
    \item $t1 = x - 1$
    \item $t2 = x \mid t1$
    \item $t3 = t2 + 1$
    \item $t4 = t3 \& x$
   \end{enumerate}
   \end{minipage}
   \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   \bf{P18}($x$): Determine if $x$ is a power of 2.
   \begin{enumerate}
    \item $t1 = -x$
    \item $t2 = x \oplus t1$
    \item $t3 = t2 < t1$
   \end{enumerate}
   \end{minipage}
   \vspace{12pt}
  
  \iffalse
   \begin{minipage}{.2\textwidth}
   \bf{P19}($x, m, k$): Exchange two fields of $x$, demarcated by $m$ and $k$.
   \begin{enumerate}
    \item $t1 = x >> k$
    \item $t2 = x \oplus t1$
    \item $t3 = t2 & m$
    \item $t4 = t3 << k$
    \item $t5 = t4 \oplus t3$
    \item $t6 = t5 \oplus x$
   \end{enumerate}
   \end{minipage}
   \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   \bf{P20}($x$): Next higher unsigned number with the same number of 1 bits.
   \begin{enumerate}
    \item $t1 = \sim x$
    \item $t2 = x \& t1$
    \item $t3 = x + t2$
    \item $t4 = x \opus t2$
    \item $t5 = t4 >> 2$
    \item $t6 = t5 / t2$
    \item $t7 = t6 \mid t3$
   \end{enumerate}
   \end{minipage}
   \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   \bf{P21}($x, a, b, c$): Cycling through 3 values $a, b, c$.
   \begin{enumerate}
    \item $t1 = x \neq c$
    \item $t2 = a \oplus c$
    \item $t3 = x \neq a$
    \item $t4 = b \oplus c$
    \item $t5 = t2 \& t2$
    \item $t6 = t3 \& t4$
    \item $t7 = t5 \oplus t6$
    \item $t8 = t7 \oplus c$
   \end{enumerate}
   \end{minipage}
\fi
   
   
   \begin{minipage}{.2\textwidth}
   {\bf P19($x, m, k$): Exchange two fields of $x$, demarcated by $m$ and $k$.}

   N/A ({\sc Kalashnikov} was unable to synthesise this program.)
   \end{minipage}
   \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   {\bf P20($x$): Next higher unsigned number with the same number of 1 bits.}

   N/A
   \end{minipage}
   \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   {\bf P21($x, a, b, c$): Cycling through 3 values $a, b, c$.}

    N/A
   \end{minipage}
   \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   {\bf P22($x$): Compute parity.}

    N/A
   \end{minipage}
   \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   {\bf P23($x$): Count number of set bits.}

    N/A
   \end{minipage}
      \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   {\bf P24($x$): Round up to next highest power of 2.}

    N/A
   \end{minipage}
   \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   {\bf P25($x, y$): Computer higher order half of $x \times y$.}

    N/A
   \end{minipage}

   \vspace{12pt}

   \begin{minipage}{.2\textwidth}
   {\bf P26($x, k$): Round $x$ up to a multiple of $2^k$.}

N/A
   \end{minipage}

      \vspace{12pt}
   
   \begin{minipage}{.2\textwidth}
   {\bf P27($x, y$): Min.}
    \begin{enumerate}
     \item $t1 = x \oplus y$
     \item $t2 = t1 \leq t2$
     \item $t3 = t1 * t2$
     \item $t4 = y \oplus t3$
    \end{enumerate}
   \end{minipage}

   
 \end{multicols}

 \caption{The integer benchmarks}
\end{figure}

\begin{figure}
 \begin{lstlisting}[language=C++]
void interchangeObs(word_t* src, word_t* dest)
{
  *src = *src ^ *dest;

  if (*src == (*src ^ *dest)) {
    *src = *src ^ *dest;

    if (*src == (*src ^ *dest)) {
      *dest = *src ^ *dest;
      
      if (*dest == (*src ^ *dest)) {
        *src = *dest ^ *src;
        return;
      } else {
        *src = *src ^ *dest;
        *dest = *src ^ *dest;
        return;
      } 
    } else
      *src = *src ^ *dest;
  }
  
  *dest = *src ^ *dest;
  *src = *src ^ *dest;

  return;
}
 \end{lstlisting}

 \caption{Benchmark 28: an obfuscated swap function}
\end{figure}

\begin{figure}
 \begin{lstlisting}[language=C++]
int mul45(int y) {
  int a=1, b=0, z=1, c=0;

  while(1) {
    if (a == 0) {
      if (b == 0) {
	y=z+y; a =!a; b=!b;c=!c;
	if (! c) break;
      } else {
	z=z+y; a=!a; b=!b; c=!c;
	if (! c) break;
      }
    } else {
      if (b == 0) { z=y << 2; a=!a; }
      else {
	z=y << 3; a=!a; b=!b; } } }

  return y;
}
	
 \end{lstlisting}

 \caption{Benchmark 29: an obfuscated function to multiply by 45}
 
\end{figure}



==> synth-complexity.tex <==
\section{Decision Procedure for Second-Order SAT}
\label{sec:complexity}

\todo{this section should contain: brief intro of finite state synthesis + the connection to 2nd order SAT (Theorem 3)}


The program synthesis problem can be informally described as follows:
given a specification, find a program which satisfies that specification for all inputs.
In order to define this problem formally, we need to identify what a specification is,
what the program we are synthesising is, and what an input is.

\subsection{General Program Synthesis}

For the general case of program synthesis, we will say that:

\begin{itemize}
 \item The program we wish to
synthesise is a Turing machine computing a total function which takes as input a natural number and
produces another natural number.
 \item A specification is a computable function $\sigma(P, x)$ whose arguments are $P$ --
the index of some Turing machine, and $x$ a natural number.
\end{itemize}

The synthesis problem is then that of finding some program $P$ such that the synthesis formula of Definition~\ref{def:synth-formula}
is true, where we introduce a function $H(P, x)$ which returns true iff the Turing machine
with index $P$ halts on input $x$.

\begin{definition}[Synthesis Formula]
 \label{def:synth-formula}
 \[
 \forall x \in \mathbb{N} . \sigma(P, x) \wedge H(P, x)
 \]
\end{definition}

The decision problem associated with program synthesis is to determine whether such a $P$
exists for a given $\sigma$.  We can see immediately
that this decision problem is equivalent to the halting problem for an oracle machine
with access to the oracle $H$.  It is a well known result that an oracle machine
cannot solve its own halting problem, and so the program synthesis problem is
undecidable even if we have access to an oracle solving the halting problem.
In other words, the general synthesis problem has Turing degree $0''$, making it
strictly harder than the halting problem for Turing machines.

In order to recover decidability, we can restrict our scope and consider a finite version of the synthesis
problem in which the programs we wish to synthesise have a finite state space
$\mathcal{S}$.  Since we require our programs to halt on all inputs, we
can identify each program $P$ with the total function $f : \mathcal{S} \to \mathcal{S}$
it computes.

\subsection{Program Encodings}
Now we turn to the problem of how to encode such finite-state programs.
For the remainder of this thesis, we will encode finite-state programs as loop-free
imperative programs consisting of a sequence of instructions, each instruction
consisting of an opcode and a tuple of operands.  The opcode specifies which
operation is to be performed and the operands are the arguments on which the
operation will be performed.  We allow an operand to be one of: a constant literal,
an input to the program, or the result of some previous instruction.  Such a program
has a natural correspondence with a combinational circuit.

A sequence of instructions is certainly a natural encoding of a program,
but we might wonder if it is the \emph{best} encoding.
We can show that for a reasonable set of instruction types (i.e.~valid opcodes), this encoding
is optimal in a sense we will now discuss.
An encoding scheme $E$ takes a function $f$ and assigns it a name $s$.  For a given ensemble
of functions $F$ we are interested in the worst-case behaviour of the encoding $E$, that is we are
interested in the quantitiy $$|E(F)| = \max \{ |E(f)| \mid f \in F \}$$
If for every encoding $E'$, we have that $$|E(F)| = |E'(F)|$$ then we say that $E$ is an \emph{optimal encoding}
for $F$.  Similarly if for every encoding $E'$, we have $$O(|E(F)|) \subseteq O(|E'(F)|)$$ we say that $E$ is
an \emph{asymptotically optimal encoding} for $F$.


\begin{lemma}[Languages with ITE are Universal and Optimal Encodings for Finite Functions]
\label{lem:ite-size}
 For an imperative programming language including instructions
 for testing equality of two values (EQ) and an if-then-else
 (ITE) instruction, any total function $f : \mathcal{S} \to \mathcal{S}$
 can be computed by a program of size $O(| \mathcal{S} | \log | \mathcal{S} |)$ bits.
\end{lemma}

\begin{proof}
The function $f$ is computed by the following program:

 \begin{verbatim}
t1 = EQ(x, 1)
t2 = ITE(t1, f(1), f(0))
t3 = EQ(x, 2)
t4 = ITE(t3, f(2), t2)
...
 \end{verbatim}

Each operand can be encoded in $\log_2 (| \mathcal{S} | + l) = \log_2 (3 \times | \mathcal{S} |)$ bits.
So each instruction can be encoded in $O(\log | \mathcal{S} |)$ bits and there are $O(|\mathcal{S}|)$
instructions in the program, so the whole program can be encoded in $O(| \mathcal{S} | \log | \mathcal{S} |)$
bits.
\end{proof}

\begin{lemma}
\label{lem:large-encoding}
 Any representation that is capable of encoding an arbitrary total function $f : \mathcal{S} \to \mathcal{S}$
 must require at least $O(| \mathcal{S} | \log | \mathcal{S} |)$ bits to encode some functions.
\end{lemma}

\begin{proof}
 There are $| \mathcal{S} |^{| \mathcal{S} |}$ total functions $f : \mathcal{S} \to \mathcal{S}$.
 Therefore by the pigeonhole principle, any encoding that can encode an arbitrary function must use
 at least $\log_2 (| \mathcal{S} |^{| \mathcal{S} |}) = O(| \mathcal{S} | \log_2 | \mathcal{S} |)$
 bits to encode some function.
\end{proof}

From Lemma~\ref{lem:ite-size} and Lemma~\ref{lem:large-encoding}, we can conclude that \emph{any}
set of instruction types that include ITE is an asymptotically optimal function encoding for total functions with
finite domains.

\subsection{Finite Program Synthesis}

To formally define the finite synthesis problem, we will require that the inputs $x$ are drawn
from some finite domain $\mathcal{D}$
and that $P$ and $\sigma$ are loop-free imperative programs.  We will allow $\sigma$
to make use of a \verb|CALL| instruction with which it can call $P$ as a subroutine.
We then define the finite-state synthesis decision problem as checking the truth of
Definition~\ref{def:finite-synth-formula}.

\begin{definition}[Finite Synthesis Formula]
 \label{def:finite-synth-formula}
\[
 \exists P . \forall x \in \mathcal{D} . \sigma(x)
\]
\end{definition}

We will now show that each instance of Definition~\ref{def:2sat} can be reduced in polynomial
time to an instance of Definition~\ref{def:finite-synth-formula}.

\begin{theorem}[Second-Order SAT is Polynomial Time Reducible to Finite Synthesis]
 Every instance of Definition~\ref{def:2sat} is polynomial time reducible to an instance
 of Definition~\ref{def:finite-synth-formula}.
\end{theorem}

\begin{proof}
 We first Skolemise the instance of definition~\ref{def:2sat} to produce an equisatisfiable
 second-order sentence with the first-order part only having universal quantifiers
 (i.e. bring the formula into Skolem normal form).  This process will have introduced
 a function symbol for each first order existentially quantified variable and taken
 linear time.  Now we just existentially quantify over the Skolem functions, which
 again takes linear time and space.
 The resulting formula is an instance of Definition~\ref{def:finite-synth-formula}.
\end{proof}

\begin{corollary}
\label{cor:finite-synth-nexp}
 Finite-state program synthesis is NEXPTIME-complete.
\end{corollary}


==> synth-fragment.tex <==

\section{Existential Second-Order Logic}

We will now digress briefly to discuss program synthesis.  This discussion
will allow us to characterise a fragment of second-order logic that has the
desirable properties of being very expressive and at the same time
restrictive enough to admit effective, automated reasoning.

Program synthesis is concerned with automatically constructing programs that
meet some specification.  We can formalise this notion with the following
second-order formula:


\begin{definition}[Synthesis Formula]
\label{def:synth-formula}
%
 \[
  \exists F . ~\forall x .\, \sigma(F, x)
 \]
%
$F : X \to Y$ ranges over computable functions, $x$ ranges over
ground terms.  The specification $\sigma: (X \to Y) \times
X \to \mathbb{B}$ is a function that returns true iff $F$ is ``correct''
when fed the input $x$.
%
\end{definition}

With this definition in hand, we can say that the program synthesis problem is
that of checking the satisfiability of Definition~\ref{def:synth-formula} and
finding a witness program $P$ (which computes $F$) if the formula is satisfiable.

In fact the correspondence between program synthesis and Definition~\ref{def:synth-formula}
goes both ways: if we have a formula $\phi$ that is of the same syntactic form as
Definition~\ref{def:synth-formula}, we can construct a program synthesis problem that is
solvable iff $\phi$ is satisfiable.  So if we had a program synthesiser, we would be
able to check satisfiability of some fragment of second-order formulae.  We will now
describe precisely the fragment of second-order logic for which satisfiability
can be reduced to program synthesis by slightly generalising Definition~\ref{def:synth-formula}.
We will refer to this fragment as the \emph{synthesis fragment}.

\begin{definition}[Generalised Synthesis Formula]
\label{def:general-synth-formula}
 \[
  \exists \vec{F} . Q_1 \vec{x_1} \ldots Q_n \vec{x_n} . \sigma(\vec{F}, \vec{x_1}, \ldots, \vec{x_n})
 \]
The functions $\vec{F}$ range over computable functions; the $\vec{x_i}$
range over vectors of ground terms; the $Q_i$ are arbitrary first order quantifiers: $\forall$ or $\exists$.
\end{definition}

Every instance of Definition~\ref{def:general-synth-formula} can be reduced to a
logically equivalent instance of Definition~\ref{def:synth-formula} by Skolemising
and adding the Skolem functions to the vector $\vec{F}$ that we quantify over.

As well as syntactic restrictions, there are semantic restrictions imposed
on formulae in the synthesis fragment.  In particular, the fragment is
implicitly parametrised by a background theory $\mathcal{T}$.
The functions $\vec{F}$ and $\sigma$ must be computable, total and
expressible in $\mathcal{T}$.

For example, if we use Peano arithmetic as our background theory, the fragment
defined by Definition~\ref{def:general-synth-formula} is the class of
$\Sigma^1_1$ formulae.  Notably, this class includes all first order formulae
with \emph{arbitrary quantifier alternation}.  Since $\Sigma^0_1$ is the
set of all recursively enumerable sets and $\Pi^0_2$ is the set of
all Turing machines that halt on all inputs (and $\Sigma^1_1$ contains
all sets $\Sigma^0_n$ and $\Pi^0_n$), it can be seen that this fragment
is rather expressive.

So we have established that the synthesis fragment can be used to model a large
class of program analysis problems,
and that if we had an automatic program synthesiser
we would be able to automatically check satisfiability of a formula
in the synthesis fragment.  In the next sections, we will
show how to build such a program synthesiser.

==> synth-icse-results-table.tex <==
\begin{tabular}{l||rr|rrc|rr}
Problem & \multicolumn{2}{c}{Random {\sc Brahma}} & \multicolumn{3}{|c}{Semibiased {\sc Brahma}} & \multicolumn{2}{|c}{\sc Kalashnikov} \\
        & Runtime & \#Lines & Runtime & \#Lines & Aut. & Runtime & \#Lines \\
\hline
\hline
p1 & 1.48s &2 &{\bf 0.80s} &2 & & 1.83s &2 \\
p2 & 7.35s &2 &4.75s &2 & & {\bf 1.49s} &2 \\
p3 & 1.60s &2 &{\bf 0.65s} &2 & & 1.60s &2 \\
p4 & 1.65s &2 &{\bf 0.86s} &2 & & 1.86s &2 \\
p5 & 3.92s &2 &2.28s &2 & & {\bf 1.98s} &2 \\
p6 & 6.22s &2 &1.64s &2 & & {\bf 1.51s} &2 \\
p7 & 1.39s &3 &{\bf 0.50s} &3 & & 4.04s &3 \\
p8 & 2.20s &3 &{\bf 1.42s} &3 & & 4.31s &3 \\
p9 & {\bf 4.95s} &3 &8.75s &3 &\xmark & 5.74s &3 \\
p10 & 13.99s &3 &{\bf 7.82s} &3 &\xmark & 9.80s &3 \\
p11 & 24.31s &3 &17.13s &3 &\xmark & {\bf 9.40s} &3 \\
p12 & 279.49s &3 &48.16s &3 &\xmark & {\bf 10.12s} &3 \\
p13 & 32.50s &4 &{\bf 9.97s} &4 &\xmark & 10.24s &{\bf 3} \\
p14 & 14.32s &4 &{\bf 6.66s} &4 &\xmark & -- &-- \\
p15 & 167.84s &4 &{\bf 18.07s} &4 &\xmark & 40.28s &4 \\
p16 & 66.93s &4 &{\bf 23.92s} &4 &\xmark & 27.41s &4 \\
p17 & 217.34s &4 &{\bf 26.51s} &4 &\xmark & 41.37s &4 \\
p18 & 228.78s &4 &{\bf 33.53s} &4 &\xmark & 35.02s &4 \\
p19 & 163.82s &4 &65.45s &4 & & {\bf 27.73s} &4 \\
p20 & 214.14s &6 &82.53s &6 &\xmark & {\bf 5.55s} &{\bf 3} \\
p21 & 1074.04s &7 &{\bf 285.56s} &7 &\xmark & -- &-- \\
p22 & -- &-- &{\bf 372.74s} &12 &\xmark & -- &-- \\
p23 & 1.38s &3 &12.12s &3 & & {\bf 1.20s} &{\bf 2} \\
p24 & 5.28s &4 &{\bf 2.96s} &4 & & 4.64s &{\bf 1} \\
\end{tabular}


==> synth-results-table.tex <==
\begin{tabular}{l||rrc|rrrc|rr|rr}
Problem & \multicolumn{3}{c}{\sc PLDI Brahma} & \multicolumn{4}{|c}{ICSE Brahma} & \multicolumn{2}{|c}{\sc Brahmikov} & \multicolumn{2}{|c}{\sc Kalashnikov} \\
        & Runtime & \#Lines & Aut. & Random & Semibiased & \#Lines & Aut. & Runtime & \#Lines & Runtime & \#Lines \\
\hline
\hline
p1 & 3.20s &{\bf 2} & & 1.48s & {\bf 0.80s} & {\bf 2} & & 117.02s &12 &1.87s &{\bf 2} \\
p2 & 3.60s &2 & & 7.35s & 4.75s & 2 & & 46.38s &12 &{\bf 3.43s} &{\bf 1} \\
p3 & 1.40s &{\bf 2} & & 1.60s & {\bf 0.65s} & {\bf 2} & & 131.06s &12 &1.92s &4 \\
p4 & 3.30s &{\bf 2} & & 1.65s & {\bf 0.86s} & {\bf 2} & & 52.13s &12 &2.22s &4 \\
p5 & {\bf 2.20s} &{\bf 2} & & 3.92s & 2.28s & {\bf 2} & & 73.60s &12 &2.82s &4 \\
p6 & 2.40s &2 & & 6.22s & {\bf 1.64s} & 2 & & 41.95s &12 &1.91s &{\bf 1} \\
p7 & 1.00s &{\bf 3} & & 1.39s & {\bf 0.50s} & {\bf 3} & & 166.56s &12 &1.91s &4 \\
p8 & {\bf 1.40s} &{\bf 3} & & 2.20s & 1.42s & {\bf 3} & & 86.30s &12 &2.39s &4 \\
p9 & 5.80s &{\bf 3} & & 4.95s & 8.75s & {\bf 3} & \xmark & 524.77s &12 &{\bf 2.03s} &4 \\
p10 & 76.10s &{\bf 3} & & 13.99s & 7.82s & {\bf 3} & \xmark & T/O &-- &{\bf 6.26s} &4 \\
p11 & 57.10s &{\bf 3} & & 24.31s & {\bf 17.13s} & {\bf 3} & \xmark & T/O &-- &34.12s &4 \\
p12 & 67.80s &{\bf 3} & & 279.49s & {\bf 48.16s} & {\bf 3} & \xmark & 534.26s &12 &T/O &-- \\
p13 & {\bf 6.20s} &{\bf 4} & & 32.50s & 9.97s & {\bf 4} & \xmark & 255.22s &12 &8.07s &{\bf 4} \\
p14 & 59.60s &{\bf 4} & & 167.84s & 18.07s & {\bf 4} & \xmark & T/O &-- &{\bf 11.12s} &{\bf 4} \\
p15 & 118.90s &4 & & 228.78s & {\bf 33.53s} & 4 & \xmark & T/O &-- &T/O &-- \\
p16 & 62.30s &4 & & 66.93s & 23.92s & 4 & \xmark & T/O &-- &{\bf 2.62s} &{\bf 2} \\
p17 & 78.10s &{\bf 4} & & 163.82s & {\bf 65.45s} & {\bf 4} & & 488.92s &12 &T/O &-- \\
p18 & 45.90s &6 & \xmark & 214.14s & 82.53s & 6 & \xmark & 311.58s &12 &{\bf 2.39s} &{\bf 4} \\
p19 & {\bf 34.70s} &6 & \xmark & N/A & N/A &-- & & T/O &-- &T/O &-- \\
p20 & {\bf 108.40s} &7 & \xmark & 1074.04s & 285.56s & 7 & \xmark & T/O &-- &T/O &-- \\
p21 & {\bf 28.30s} &8 & \xmark & N/A & N/A &-- & & T/O &-- &63.22s &{\bf 3} \\
p22 & {\bf 279.00s} &{\bf 8} & \xmark & N/A & N/A &-- & & T/O &-- &T/O &-- \\
p23 & {\bf 1668.00s} &10 & \xmark & N/A & N/A &-- & & T/O &-- &T/O &-- \\
p24 & {\bf 224.90s} &12 & \xmark & T/O & 372.74s & 12 & \xmark & T/O &-- &T/O &-- \\
p25 & {\bf 2778.70s} &16 & \xmark & N/A & N/A &-- & & T/O &-- &T/O &-- \\
p26 & N/A &-- & & 14.32s & 6.66s & 4 & \xmark & T/O &-- &{\bf 2.57s} &{\bf 0} \\
p27 & N/A &-- & & 217.34s & 26.51s & {\bf 4} & \xmark & T/O &-- &{\bf 1.96s} &{\bf 4} \\
p28 & N/A &-- & & {\bf 1.38s} & 24.24s & 3 & \xmark & T/O &-- &1.93s &{\bf 2} \\
p29 & N/A &-- & & 5.28s & 5.92s & 4 & \xmark & T/O &-- &{\bf 3.18s} &{\bf 1} \\
\end{tabular}


==> synth-sat.tex <==
\section{Second-Order SAT}
\label{sec:sat}

We define the second-order SAT problem as that of checking whether the following formula is satisfiable:

\begin{definition}[Second-Order SAT]
 \[
  \exists P . \forall x \in \mathcal{B}^n . \sigma(P, x)
 \]
\end{definition}

Here $\sigma$ and $P$ are loop-free C programs and $x$ is a vector of $n$ Boolean variables.
Since $n$ is at most linear in the length of $\sigma$ (which we take to be our input),
the size of $\mathcal{B}^n$ is $O(2^|\sigma|)$ and so by Fagin's theorem the decision
problem is NEXPTIME-complete.
